One For All & All For One: Bypassing Hyperparameter Tuning with Model Averaging For Cross-Lingual Transfer

Multilingual language models enable zero-shot cross-lingual transfer (ZS-XLT): fine-tuned on sizable source-language task data, they perform the task in target languages without labeled instances. The effectiveness of ZS-XLT hinges on the linguistic proximity between languages and the amount of pretraining data for a language. Because of this, model selection based on source-language validation is unreliable: it picks model snapshots with suboptimal target-language performance. As a remedy, some work optimizes ZS-XLT by extensively tuning hyperparameters: the follow-up work then routinely struggles to replicate the original results. Other work searches over narrower hyperparameter grids, reporting substantially lower performance. In this work, we therefore propose an unsupervised evaluation protocol for ZS-XLT that decouples performance maximization from hyperparameter tuning. As a robust and more transparent alternative to extensive hyperparameter tuning, we propose to accumulatively average snapshots from different runs into a single model. We run broad ZS-XLT experiments on both higher-level semantic tasks (NLI, extractive QA) and a lower-level token classification task (NER) and find that conventional model selection based on source-language validation quickly plateaus to suboptimal ZS-XLT performance. On the other hand, our accumulative run-by-run averaging of models trained with different hyperparameters boosts ZS-XLT performance and closely correlates with "oracle" ZS-XLT, i.e., model selection based on target-language validation performance.

==> backup_relevant_work.tex <==
% \sparagraph{\xlt}
% MMTs such as mBERT \citep{devlin-etal-2019-bert}, XLM-\{R,V\} \citep{conneau-etal-xlmr, fair-xlmv}, or mT5 \citep{xue-etal-2021-mt5} are pretrained on language modelling on vast corpora encompassing 100+ languages.
% Such pretraining semantically aligns representation spaces across languages to enable \xlt \citep{Cao2020Multilingual,hu2020xtreme}.
% The typological proximity between and the degree of coverage in pretraining of the source and target language nevertheless primarily determine the quality and stability of \xlt \citep{lauscher-etal-2020-zero}.
% Previous work therefore intends to better calibrate source and target language representation sub-spaces to improve \xlt.
% Continued bilingual source and target language modelling facilitates \zsxlt without supervision \cite{wu-etal-2022-zero,parovic-etal-2022-bad}.
% Dictionaries or parallel sentences underpin supervised objectives to align language sub-spaces \citep{wu-dredze-2020-explicit, hu-etal-2021-explicit}.
% Such post-hoc cross-lingual refinement nonetheless commonly necessitates potentially expensive compute resources or external data (e.g. parallel sentences or target-language annotations), inhibiting the broader application across languages, domains, and tasks \citep{ponti-etal-2019-modeling}.
% 
% \sparagraph{Averaging model weights}
% Averaging weights of models has proven effective across numerous domains such as computer vision \citep{huang2017snapshot,pmlr-v162-wortsman22a}, machine translation \citep{vaswani2017nips,gao-etal-2022-revisiting} and recently NLU \citep{wang-etal-2022-adamix,schmidt2023free}.\\
% `Model soups' compose a model by plainly averaging the snapshots that perform best on the validation set of $k$ training runs with varying hyperparameter configurations. `Souping' successfully boosts performance in image though not sequence classification tasks \cite{pmlr-v162-wortsman22a}.\footnote{See Appendix J.5 of \citet{pmlr-v162-wortsman22a}.}
% `Adamix' concurrently fine-tunes 4 adapters with alignment constraints \citep{wang-etal-2022-adamix} that are averaged prior to inference. While the approach achieves consistent gains on GLUE~\citep{wang2018glue}, it increases training time two to ten-fold. The authors also show that averaging aligned task-adapters performs better than ordinary logit ensembling.
% \citet{schmidt2023free} enables `souping' for sizable gains in \xlt as follows.
% The authors first customarily fine-tune an MMT on labelled data. They then extract from the initial run and freeze the task head for repeated training iterations, which aligns snapshots for souping. Fine-tuning models on randomly initialized heads otherwise yields sets of parameters geared to orthogonal output, i.e. misaligned, representation spaces.
% 
% We adopt the approach of \citet{schmidt2023free} and empirically illustrate that, in hyperparameter tuning, shallow strategies to average snapshots from the accrued runs perform on par or better than the best individual model.
% \ra therein frequently reduce the need for model selection. Model averaging thus alleviates oscillations from varying hyperparameters and constitutes an evaluation protocol that results in strong and fair baselines.
